Enhancing Fine-Grained Spatial Grounding in 3D CT Report Generation via Discriminative Guidance

Vision--language models (VLMs) for radiology report generation (RRG) can produce long-form chest CT reports from volumetric scans and show strong potential to improve radiology workflow efficiency and consistency. However, existing methods face two key limitations: (i) training supervision is often coarse, aligning a whole CT volume with a full free-text report without explicit alignment for fine-grained attributes or pathology locations; and (ii) evaluation is typically holistic (lexical overlap, entity matching, or LLM-as-a-judge scores) and not diagnostic for spatial grounding. We propose \emph{Discriminative Cue-Prompting with Prompt Dropout (DCP-PD)}, a plug-and-play framework that distills fine-grained cues from free-text reports and uses them to guide report generation while mitigating shortcut reliance via prompt dropout. DCP-PD achieves state-of-the-art performance on CT-RATE, improving macro F1 from $=0.501$ to $0.603$ (20% relative), and substantially boosts out-of-distribution performance on Rad-ChestCT from F1 $=0.266$ to $0.503$ (89% relative). Finally, we introduce a hierarchical, location-aware question-set protocol (presence $\rightarrow$ laterality $\rightarrow$ lobe) to directly assess pathology-location grounding, showing that fine-grained spatial localization remains challenging even for models that score highly on current benchmarks.

==> Sections/main/discussion.tex <==
% \noindent\textbf{Prompt-based conditioning via pre-prompts.}
% Our results suggest that classifier-derived \emph{pre-prompts} offer a simple and effective mechanism to condition long-form chest CT report generation. At the same time, incorporating ground-truth-derived cues during training requires care: the model can over-rely on these cues and learn shortcut behaviors that reduce visual grounding. We find that prompt dropout is a practical mitigation that improves robustness by preventing unconditional dependence on the pre-prompt, but it introduces a trade-off. Stronger dropout can weaken controllability and, in some cases, increase hallucination risk when the model attempts to fill in missing cues without sufficient visual evidence.

% A key advantage of pre-prompts is \emph{model-agnostic scalability}. Since the generation model only consumes the textual cues, improvements in the upstream discriminative component (e.g., better classifiers, calibrated thresholds, stronger ensembles) translate directly into stronger conditioning and better generation quality, without retraining the generator. This property also aligns naturally with boosting-style strategies: progressively improving or combining discriminative predictors yields progressively better conditioning signals.

% Finally, pre-prompts generalize beyond global findings. Because they are expressed in language, the same mechanism can scale to richer fact types, such as location-conditioned cues (e.g., laterality and lobar findings). This enables controllable generation at different granularity levels and provides a lightweight path toward more spatially grounded reports, as long as the underlying cues are reliable.

% \vspace{0.3em}
% \noindent\textbf{Evaluation beyond presence/absence and holistic metrics.}
% Chest CT report generation has seen diverse architectures and substantial effort toward grounding, yet common evaluations often fail to reflect \emph{where} a finding is described, or whether a model is correct at finer spatial granularity. In particular, while GREEN, originally developed for chest X-ray reports, can sometimes capture coarse consistency (and may weakly reflect location), its LLM-as-a-judge nature provides limited transparency and struggles to reveal detailed error patterns. Moreover, we observe that directly applying GREEN to chest CT can be unreliable under true-negative dominance: when many findings are absent in typical CT reports, the score can be inflated and obscure clinically meaningful mistakes.

% One possible direction is to leverage structured validation targets in which section-wise significance labels are available, potentially enabling an LLM-based evaluator to weight clinically important sections more heavily. However, such an evaluator should ultimately be validated against radiologist judgment; we leave this for future work.

% As a practical compromise, our LLM parsing agent paired with \emph{predefined discriminative question sets} provides an interpretable and extensible evaluation interface. By expanding questions from global presence to laterality and lobar location, we obtain finer-grained signals and expose patterns that are difficult to diagnose with holistic metrics alone. We encourage future report-generation benchmarks to incorporate similar question-set evaluations, and to further develop clinically meaningful, location-aware question designs that better align evaluation with grounding objectives.

% -------------here

% \subsection{Distilling Discriminative Signals via Pre-Prompt Conditioning}
% \noindent\textbf{Discriminative models are stronger than VLMs and flexible.}
% Discriminative models are typically stronger than generative VLMs for detection tasks because they are trained with direct supervision and optimized explicitly for classification. They are also flexible: supervision can be mined from free-form radiology reports on demand, enabling scalable expansion to new findings and finer-grained attributes without dense manual annotation.

% \noindent\textbf{Discriminative Pre-Prompt Conditioning is an effective integration mechanism.}
% Discriminative pre-prompt conditioning is a simple and effective way to integrate discriminative strengths into VLM generation by converting classifier outputs into language cues and prepending them to the prompt, enabling transferring discriminative evidence into language generation without architectural modification.

% \noindent\textbf{Shortcut risk; dropout is a trade-off.}
% When training with ground-truth-derived cues, the model may over-rely on the pre-prompt and learn shortcuts that reduce visual grounding. Prompt dropout improves robustness by discouraging unconditional dependence on the cue, but stronger dropout can weaken controllability and reduce the performance gains provided by the discriminative cue.

% \noindent\textbf{Model-agnostic and scalable.}
% Pre-prompting depends only on the cue content, not the generator architecture. As the upstream discriminative component improves (e.g., stronger classifiers, calibration, ensembling), the cues become more reliable and generation quality can improve accordingly, consistent with boosting-style intuition.

% \noindent\textbf{Scales to richer conditioned facts.}
% Because cues are expressed in language, the same mechanism extends beyond global findings to any fact type where reliable external predictors exist. In this paper, we instantiate this with location-conditioned cues (laterality and lobar findings), enabling finer-grained control when the underlying cues are accurate.

% \subsection{Evaluation for Spatial Grounding}
% \noindent\textbf{Grounding progress is under-measured.}
% Chest CT report generation has made substantial progress on grounding, yet common evaluations often emphasize presence/absence or holistic report scores and do not reliably expose where a model is correct or wrong spatially.

% \noindent\textbf{GREEN is informative but limited for chest CT.}
% Although GREEN (developed for chest X-ray) can capture coarse consistency and sometimes reflects location, its LLM-as-a-judge nature offers limited transparency and struggles to reveal fine-grained error patterns. We also observe failure modes under true-negative dominance in chest CT, where many absent findings can inflate scores and mask clinically meaningful mistakes.

% \noindent\textbf{Significance-aware judging is promising but needs radiologist validation.}
% A potential direction is to use structured validation targets with section-wise significance labels to encourage evaluators to emphasize clinically important content. Such evaluators should be validated against radiologist judgments; we leave this as future work.

% \noindent\textbf{Question-set parsing is a practical compromise.}
% Our LLM parsing agent coupled with predefined discriminative question sets yields interpretable and extensible signals. Expanding from global presence to laterality and lobar questions provides finer-grained diagnostics and reveals patterns not captured by holistic metrics. We encourage future work to expand question sets toward more clinically meaningful, location-aware evaluation.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\columnwidth]{Sections/figs/case_study.pdf}
  \caption{\textbf{Case study of structured report generation with classifier-guided prompts.}
  Left: two axial CT slices from the test set highlighting lung nodules, with human-annotated nodule masks (ReXGroundingCT) overlaid together with a bilateral lung mask.
  Right: comparison of \textit{Structured} (no CLS guidance), \textit{Structured w/ CLS-Guided}, and \textit{Ground Truth} reports.
  CLS guidance yields a more specific and accurate description (e.g., millimetric nonspecific nodules in both lungs), improving alignment with the ground truth compared to the unguided baseline.}
  \label{fig:case_study}
\end{figure}





